Predicting Anti-Asian Hateful Users on Twitter during COVID-19

We investigate predictors of anti-Asian hate among Twitter users throughout COVID-19. With the rise of xenophobia and polarization that has accompanied widespread social media usage in many nations, online hate has become a major social issue, attracting many researchers. Here, we apply natural language processing techniques to characterize social media users who began to post anti-Asian hate messages during COVID-19. We compare two user groups -- those who posted anti-Asian slurs and those who did not -- with respect to a rich set of features measured with data prior to COVID-19 and show that it is possible to predict who later publicly posted anti-Asian slurs. Our analysis of predictive features underlines the potential impact of news media and information sources that report on online hate and calls for further investigation into the role of polarized communication networks and news media.

==> twitter_activity.tex <==
\subsubsection{Twitter Activity} 
The first noticeable difference between hateful users and references users is their level of activity in terms of the number of written tweets after COVID-19. 
% Figure~\ref{fig:hist_perc_increase} shows the distribution of the percentage increase of the average daily number of tweets per user after COVID-19 compared with before COVID-19. 
% \begin{figure}[h!]
% \centering
% \includegraphics[width=.75\columnwidth]{figures/hist_perc_increase}
% % \label{fig:hist_perc_increase}
% % \subfigure[Overtime]{\includegraphics[width=.3\columnwidth]{figures/overtime_ntweets_hatespeakers_vs_referenceusers}\label{fig:ntweets_overtime}}
% % \subfigure[00]{\includegraphics[width=.3\columnwidth]{figures/hist_perc_increase}\label{fig:hist_perc_increase}}
% % \subfigure[00]{\includegraphics[width=.3\columnwidth]{figures/bootstrap_perc_increase_avg}\label{fig:bootstrap_perc_increase_avg}}
% \caption{Percentage increase of number of tweets after COVID-19 per user compared with before COVID-19.} 
% \label{fig:hist_perc_increase}
% \end{figure}
On average, both user groups increased their activities, and the increase is larger for hateful users. 
We evaluate the statistical significance of the increase by using bootstrapping method. The bootstrapped average percent increase among hateful users is much higher than that of reference users:
$90.12\,\%$ ($\pm 0.419\,\%$, 95\% CI) versus $24.52\,\%$ ($\pm 0.107\,\%$, 95\% CI). The results are based on 1,000 bootstrapped samples.  Furthermore, we observe that the increase in activity after COVID-19 is driven more by those High-level hateful users than Low-level ones.  The bootstrapped average percent increase among High- and Low-level hateful users are $118.97\,\%$ ($\pm 0.977\,\%$, 95\% CI) and $77.22\,\%$ ($\pm 0.381\,\%$, 95\% CI), respectively. 

